Flow Metrics on Graphs

Given a graph with non-negative edge weights, there are various ways to interpret the edge weights and induce a metric on the vertices of the graph. A few examples are shortest-path, when interpreting the weights as lengths; resistance distance, when thinking of the graph as an electrical network and the weights are resistances; and the inverse of minimum $st$-cut, when thinking of the weights as capacities. It is known that the 3 above-mentioned metrics can all be derived from flows, when formalizing them as convex optimization problems. This key observation led us to studying a family of metrics that are derived from flows, which we call flow metrics, that gives a natural interpolation between the above metrics using a parameter $p$. We make the first steps in studying the flow metrics, and mainly focus on two aspects: (a) understanding basic properties of the flow metrics, either as an optimization problem (e.g. finding relations between the flow problem and the dual potential problem) and as a metric function (e.g. understanding their structure and geometry); and (b) considering methods for reducing the size of graphs, either by removing vertices or edges while approximating the flow metrics, and thus attaining a smaller instance that can be used to accelerate running time of algorithms and reduce their storage requirements. Our main result is a lower bound for the number of edges required for a resistance sparsifier in the worst case. Furthermore, we present a method for reducing the number of edges in a graph while approximating the flow metrics, by utilizing a method of [Cohen and Peng, 2015] for reducing the size of matrices. In addition, we show that the flow metrics satisfy a stronger version of the triangle inequality, which gives some information about their structure and geometry.

==> chapters/properties_of_flow_metrics/equivalent_definitions.tex <==




Moreover, note that we can
switch between
the constraints and the objectives
of problem (\ref{eq: dual of the flow problem})
and get the following.
\begin{equation}\label{eq: bar(d)_p metric as convex optimization problem}
    \begin{array}{lllr}
        \bar{d}_p(u,v) = & \min &  \norm{WB\phi}_q\\
         & \text{s.t. }&\prs{\chi_u-\chi_v}^T\phi=1&
    \end{array}
\end{equation}
Now, we can see that,
\begin{claim}
\[
\bar{d}_p=\frac{1}{\widetilde{d}_p}
\]
\end{claim}
\begin{proof}
Indeed, suppose that $\phi^*$ is a solution to
(\ref{eq: bar(d)_p metric as convex optimization problem}).
Define 
\[
    \widetilde{\phi} = \frac{\phi^*}{\norm{WB\phi^*}_q}
\]
Thus, we can see that
\[
    \widetilde{d}_p(u,v)\geq \prs{\chi_u-\chi_v}^T\widetilde{\phi}
    =\prs{\chi_u-\chi_v}^T \frac{\phi^*}{\norm{WB\phi^*}_q}
    = \frac{1}{\norm{WB\phi^*}_q}=\frac{1}{\bar{d}_p(u,v)}
\]
Similarly we can show that $\bar{d}_p(u,v)\leq\frac{1}{\widetilde{d}_p(u,v)}$,
which will lead us to the desired conclusion.
\end{proof}

Moreover, we have the following.
\begin{claim}
Let $G=(V,E,w)$ be a graph, let $p\in[1,\infty]$,
let $q=\frac{p}{p-1}$ be the H\"older conjugate of $p$.
Then,
\begin{equation}
    \forall s,t\in V,\quad
    \widetilde{d}_p(s,t) = \max_{\substack{\phi\in \R^V\\\phi\notin\text{span}\curprs{\OneVec}}}
    \frac{\prs{\chi_s-\chi_t}^T\phi}{\norm{WB\phi}_q}
\end{equation}
\end{claim}
Hence, since $d_p=\widetilde{d}_p$,
we get another characterization of the flow metrics.
\begin{proof}
Fix some $s\neq t\in V$.
First, note that for every $\phi\in\R^V$
such that $\norm{WB\phi}_q=1$
it holds that $\phi\notin\text{span}\curprs{\OneVec}$
(otherwise the norm would have been 0 since
$\text{ker}B=\text{span}\curprs{\OneVec}$)
and $\prs{\chi_s-\chi_t}\phi = \frac{\prs{\chi_s-\chi_t}\phi}{\norm{WB\phi}_q}$.
Hence, it is immediate that
\begin{equation}
    \widetilde{d}_p(s,t) \leq \max_{\substack{\phi\in \R^V\\\phi\notin\text{span}\curprs{\OneVec}}}
    \frac{\prs{\chi_s-\chi_t}^T\phi}{\norm{WB\phi}_q}
\end{equation}
On the other hand, let
\[
    \phi^*\in\argmax{\substack{\phi\in \R^V\\\phi\notin\text{span}\curprs{\OneVec}}}\frac{\prs{\chi_s-\chi_t}^T\phi}{\norm{WB\phi}_q},
\]
and define $\widetilde{\phi} = \frac{\phi^*}{\norm{WB\phi^*}_q}$.
It is easy to see that
$\widetilde{\phi}\notin\text{span}\curprs{\OneVec}$,
$\norm{WB\widetilde{\phi}}_q=1$,
and moreover,
\begin{equation}
    \begin{split}
        \widetilde{d}_p(s,t) & \geq \prs{\chi_s-\chi_t}^T\widetilde{\phi}
        = \frac{\prs{\chi_s-\chi_t}^T\phi^*}{\norm{WB{\phi^*}}_q}
        =  \max_{\substack{\phi\in \R^V\\\phi\notin\text{span}\curprs{\OneVec}}}
    \frac{\prs{\chi_s-\chi_t}^T\phi}{\norm{WB\phi}_q}.
    \end{split}
\end{equation}
\end{proof}
\begin{comment}
\begin{proof}
First we remark that it is enough 
to discuss $\varphi\in\R^V$ such that $\varphi_u-\varphi_v=1$,
e.g. we will show that the following holds.
\[
    \max_{\substack{\varphi\in \R^V\\ \varphi\notin\text{span}\curprs{\OneVec}}} \curprs{\frac{\abs{\varphi_u-\varphi_v}}{\prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\varphi_x-\varphi_y}^q}^{1/q}}}
    = 
    \max_{\varphi_u-\varphi_v=1}
    \curprs{\frac{\abs{\varphi_u-\varphi_v}}{\prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\varphi_x-\varphi_y}^q}^{1/q}}}
\]
Indeed, fix some $\phi\in\R^V$,
and define $\varphi\in \R^V$
as follows
\[
    \forall x\in V:\quad \varphi_x= \frac{\phi_x-\phi_v}{\phi_u-\phi_v}
\]
Thus, we get that $\varphi_u-\varphi_v=1$,
and
\begin{align*}
    \frac{\abs{\varphi_u-\varphi_v}}{\prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\varphi_x-\varphi_y}^q}^{1/q}}
    & = \frac{\abs{\frac{\phi_u-\phi_v}{\phi_u-\phi_v}-
    \frac{\phi_v-\phi_v}{\phi_u-\phi_v}}}{\prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\frac{\phi_x-\phi_v}{\phi_u-\phi_v}
    -\frac{\phi_y-\phi_v}{\phi_u-\phi_v}}^q}^{1/q}}\\
    & = \frac{\abs{1-0}}{
    \frac{1}{\abs{\phi_u-\phi_v}}
    \prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\phi_x-\phi_v
    -\prs{\phi_y-\phi_v}}^q}^{1/q}}\\
    & = \frac{\abs{\phi_u-\phi_v}}{
    \prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\phi_x
    -\phi_y}^q}^{1/q}}\\
\end{align*}

Now, we can see that
\begin{align*}
    \max_{\substack{\varphi\in \R^V\\ \varphi\notin\text{span}\curprs{\OneVec}}} \curprs{\frac{\abs{\varphi_u-\varphi_v}}{\prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\varphi_x-\varphi_y}^q}^{1/q}}}
    & =
    \max_{\varphi_u-\varphi_v=1}
    \curprs{\frac{\abs{\varphi_u-\varphi_v}}{\prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\varphi_x-\varphi_y}^q}^{1/q}}}\\
    & = 
    \max_{\varphi_u-\varphi_v=1}
    \curprs{\frac{1}{\prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\varphi_x-\varphi_y}^q}^{1/q}}}\\
    & = \frac{1}{\min_{\varphi_u-\varphi_v=1}\curprs{\prs{\sum_{xy\in E}w(xy)^q\cdot\abs{\varphi_x-\varphi_y}^q}^{1/q}}}\\
    & = \frac{1}{\Bar{d}_p(u,v)}\\
    & = d_p(u,v)
\end{align*}

\end{proof}
\end{comment}




\textbf{***TODO: add some words about Laplacians and p-Laplacians?...
What aboud KKT conditions? present it as a fact and mention that it yields a generalization of Ohm's law?}





\begin{claim}\label{claim: closed form solution for d_p}
Let $G=(V,E,w)$ be a graph with signed edge-vertex incidence matrix $B$,
let $p\in (1,\infty)$ with H\"older conjugate $q$, 
let $s,t\in V$, let $f\in\R^E$
and $\varphi\in \R^V$ such that
\begin{align}
    &&&& B^Tf & = \chi_s-\chi_t,\\
    &\text{and }\forall xy\in E, &&& 
    \varphi_x-\varphi_y & = \frac{f(xy)\abs{f(xy)}^{p-2}}{w(xy)^p}
    \\
    &\text{or equivalently,} &&&
    f(xy) & = w(xy)^q\prs{\varphi_x-\varphi_y}\abs{\varphi_x-\varphi_y}^{q-2}.
\end{align}
Then, $f$ is an optimal flow for $d_p$
and $\varphi$ is an optimal potentials function for $\bar{d}_p$ .
Moreover,
\begin{equation}
    d_p(s,t) = \prs{\varphi_s-\varphi_t}^{1/p}
\end{equation}
\end{claim}
First, note that the two definitions  are indeed equivalent since by plugging one into the other
we see that,
\begin{equation}
    \begin{split}
        \varphi_x-\varphi_y & = \frac{f(xy)\abs{f(xy)}^{p-2}}{w(xy)^p}\\
        & = \frac{\prs{w(xy)^q\prs{\varphi_x-\varphi_y}\abs{\varphi_x-\varphi_y}^{q-2}}\abs{w(xy)^q\prs{\varphi_x-\varphi_y}\abs{\varphi_x-\varphi_y}^{q-2}}^{p-2}}{w(xy)^p}\\
        & = w(xy)^{q+q(p-2)-p}
        \cdot \prs{\varphi_x-\varphi_y}
        \cdot\abs{\varphi_x-\varphi_y}^{q-2+(q-1)(p-2)}\\
        & = \prs{\varphi_x-\varphi_y}
        \cdot w(xy)^{q(p-1)-p}
        \cdot\abs{\varphi_x-\varphi_y}^{(q-1)(p-1)-1}\\
        & = \prs{\varphi_x-\varphi_y}
        \cdot w(xy)^{\frac{p(p-1)}{p-1}-p}
        \cdot\abs{\varphi_x-\varphi_y}^{\frac{p-1}{p-1}-1}\\
        & =  \varphi_x-\varphi_y
    \end{split}
\end{equation}

\begin{proof}
On the one hand, we can see that
\begin{equation}
    \begin{split}
        d_p(s,t)^p & \leq \sum_{e\in E}\abs{\frac{f(e)}{w(e)}}^p\\
        & = \sum_{xy\in E}f(xy)\cdot\frac{f(xy)\abs{f(xy)}^{p-2}}{w(xy)^p}\\
        & = \sum_{xy\in E}f(xy)\prs{\varphi_x-\varphi_y}\\
        & = f^TB\varphi\\
        & = \prs{B^Tf}^T\varphi\\
        & = \prs{\chi_s-\chi_t}^T\varphi\\
        & = \varphi_s-\varphi_t
    \end{split}
\end{equation}
Note that $\abs{f(xy)\prs{\varphi_x-\varphi_y}}=f(xy)\prs{\varphi_x-\varphi_y}$
since by definition they both have the same sign.
Similarly,
\begin{equation}
    \begin{split}
        \norm{WB\varphi}_q^q & = \sum_{xy\in E}w(xy)^q\abs{\varphi_x-\varphi_y}^q\\
        & = \sum_{xy\in E}f(xy)\prs{\varphi_x-\varphi_y}\\
        & = \varphi_s-\varphi_t
    \end{split}
\end{equation}
Thus.
\begin{equation}
    \begin{split}
        \prs{\varphi_s-\varphi_t}^{1/p}\geq d_p(s,t) & \geq \frac{\varphi_s-\varphi_t}{\norm{WB\varphi}_q}\\
        & = \frac{\varphi_s-\varphi_t}{\prs{\varphi_s-\varphi_t}^{1/q}}\\
        & = \prs{\varphi_s-\varphi_t}^{1/p}
    \end{split}
\end{equation}

\end{proof}

\begin{comment}
\subsection{Basic Properties of the Flow Metrics}
Recall that in $p$-norms we know the following bound.
\begin{proposition}\label{prop: connection between different l_p norms}
Let $1\leq p \leq {p'} \leq \infty$, let $x\in\R^n$, then
\[
    \norm{x}_{p'}\leq\norm{x}_p\leq n^{1/p-1/{p'}}\norm{x}_{p'}
\]
\end{proposition}
We can use this bound in order to reach the following conclusion.
\begin{claim}\label{claim: simple connection between different d_p metrics}
Let $G=(V,E)$ be a graph over $|V|=n$ vertices.
Let $1\leq p \leq {p'} \leq\infty$, and let $s,t\in V$.
Then
\[
    d_{p'}(s,t)\leq d_p(s,t)\leq \abs{E}^{1/p-1/{p'}}d_{p'}(s,t)
\]
\end{claim}
Before we start the proof we will need some notation.

\begin{definition}
Let $G=(V,E)$ be a graph, let $p\geq 1$, let $d_p$ be the corresponding
flow metric, and let $s,t\in V$.
Then we will denote by $f_{p,(s,t)}^{*}$ be a unit flow from $s$
to $t$ that satisfies
\[
    \norm{W^{-1}{f_{p,(s,t)}^*}}_p=d_p(s,t)
\]
In other words, it is the unit flow that minimizes the $\ell_p$ load
over all the possible unit flows from $s$ to $t$.
\end{definition}
Now we can prove Claim \ref{claim: simple connection between different d_p metrics}.
\begin{proof}
Let $G=(V,E)$ be a graph, let $1\leq p\leq {p'}\leq \infty$,
and let $s,t\in V$.
Then we can see that on the one hand,
\begin{align*}
    d_p(s,t) & = \norm{W^{-1}{f^*_{p,(s,t)}}}_p
    &&\text{definition of }f^*_{p,(s,t)}\\
    &\leq \norm{W^{-1}{f^*_{{p'},(s,t)}}}_p
    &&\text{definition of }d_p\\
    & \leq \abs{E}^{1/p-1/{p'}}\norm{W^{-1}{f^*_{{p'},(s,t)}}}_{p'}
    &&\text{Proposition \ref{prop: connection between different l_p norms}}\\
    & = \abs{E}^{1/p-1/{p'}}d_{p'}(s,t)
    &&\text{definition of }f^*_{{p'},(s,t)}
\end{align*}
and on the other hand we have
\begin{align*}
    d_{p'}(s,t) & = \norm{W^{-1}{f^*_{{p'},(s,t)}}}_{p'}
    &&\text{definition of }f^*_{{p'},(s,t)}\\
    &\leq \norm{W^{-1}{f^*_{p,(s,t)}}}_{p'}
    &&\text{definition of }d_{p'}\\
    & \leq\norm{W^{-1}{f^*_{p,(s,t)}}}_p
    &&\text{Proposition \ref{prop: connection between different l_p norms}}\\
    & = d_p(s,t)
    &&\text{definition of }f^*_{p,(s,t)}
\end{align*}
The proof is finished.
\end{proof}
As a consequence, we have the following corollary.
\begin{corollary}\label{corl: large p is essentialy infinity}
Let $G=(V,E)$ be a graph over $n=|V|$ vertices, let $\varepsilon>0$,
and suppose
that $p=\Omega\prs{\varepsilon^{-1}\cdot \log n}$.
Then,
\begin{equation}
    \forall s,t\in V,\quad
    d_\infty(s,t)\leq d_p(s,t)\leq (1+\varepsilon)d_\infty(s,t).
\end{equation}
\end{corollary}
\begin{proof}
By Claim \ref{claim: simple connection between different d_p metrics},
we have
\begin{equation}\label{eq: we know from connection between d_p and d_inf}
    d_\infty\leq d_p\leq |E|^{1/p}d_\infty.
\end{equation}
But it is easy to see that
\begin{equation}
    |E|^{1/p} = e^{\frac{1}{p}\log |E|}.
\end{equation}
Hence, for $p=\Omega\prs{\varepsilon^{-1}\log n}$ we get
that in the above equation we have
\begin{equation}
    |E|^{1/p} \leq e^{\varepsilon}\approx 1+\varepsilon.
\end{equation}
Thus, plugging this into \ref{eq: we know from connection between d_p and d_inf}
we get
\begin{equation}
    d_\infty \leq d_p \leq (1+\varepsilon)\cdot d_\infty.
\end{equation}
\end{proof}
\begin{corollary}\label{corl: connection between d_p metric and the 3 special cases}
Let $G=(V,E)$ be a graph, let $p\geq 1$,  let $d_p$ be the corresponding
flow metric. Then,
\begin{enumerate}
    \item   $d_p \stackrel{|E|}{\hookrightarrow}\ell_1,\ell_\infty$,
            because we have
            \[
                \forall s,t\in V,\quad \abs{E}^{-1}d_1(s,t)\leq d_p(s,t)\leq d_1(s,t)
            \]
            and $d_1\hookrightarrow \ell_1,\ell_\infty$.
    \item   If $p\geq 2$, we have
            $d_p \stackrel{{|E|^{1/2}}}{\hookrightarrow}\ell_2$,
            because we have
            \[
                \forall s,t\in V,\quad \abs{E}^{-1/2}d_2(s,t)\leq d_p(s,t)\leq d_2(s,t)
            \]
            and $d_2\hookrightarrow \ell_2$.
    \item   $d_p \stackrel{{|E|^{1/p}}}{\hookrightarrow}\ell_2$,
            because we have
            \[
                \forall s,t\in V,\quad d_\infty(s,t)\leq d_p(s,t)\leq \abs{E}^{1/p} d_\infty (s,t)
            \]
            and $d_\infty\hookrightarrow \ell_2$.
\end{enumerate}
\end{corollary}
We remark that the above inequalities are tight.
Consider a graph $G$ that consists of 2 vertices $s$ and $t$,
and $m$
parallel (unweighted) edges that connect between them.
Then it is easy to see that for any $p$ we have  $d_p(s,t)=m^{(1-p)/p}$.
plugging this into the above inequalities will
give equality in the RHS for $p=1,2$, (in the third
inequality we will have equality for any $p$)
and we will have equality with the LHS as $p\rightarrow\infty$.

Another conclusion that follows from the above is the following
(follows from case 3).
\begin{corollary}\label{corl: large p is essentialy infinity}
Let $G=(V,E)$ be a graph over $n=|V|$ vertices, let $\varepsilon>0$,
and suppose
that $p=\Omega\prs{\varepsilon^{-1}\cdot \log n}$,
then the corresponding $d_p$  metric over $G$
admits an embedding of distortion $1+\varepsilon$
into $\ell_2$.
\end{corollary}
\begin{proof}
By case 3 from corollary \ref{corl: connection between d_p metric and the 3 special cases},
we have
\begin{equation}\label{eq: we know from connection between d_p and d_inf}
    d_\infty\leq d_p\leq |E|^{1/p}d_\infty
\end{equation}
But it is easy to see that
\begin{equation}
    |E|^{1/p} = e^{\frac{1}{p}\log |E|}
\end{equation}
Hence, for $p=\Omega\prs{\varepsilon^{-1}\log n}$ we get
that in the above equation we have
\begin{equation}
    |E|^{1/p} \leq e^{\varepsilon}\approx 1+\varepsilon
\end{equation}
Thus, plugging this into \ref{eq: we know from connection between d_p and d_inf}
we get
\[
    d_\infty \leq d_p \leq (1+\varepsilon)\cdot d_\infty
\]
Which concludes the proof since $d_\infty$ admits an isometric embedding
into $\ell_2$.
\end{proof}
\end{comment}
%TODO: is this part gonna enter the thesis? maybe mention in the appendix?
\begin{comment}
\subsubsection{An extension of a known lemma}
For a set of vertices $U\subset V$, denote
$\gamma_{eff}(U)=\max_{x,y\in U}\Reff(x,y)$.
Madry, Straszak, and Tarnawski \cite{madry2014fast}
showed the following lemma.
\begin{lemma}\label{lemma: small cut from Madry}
Let $U,U'\subset V$ be disjoint sets in a graph $G$ having at most $m$
edges, let $p\in[1,\infty)$, let $u\in U$ and $u'\in U'$.
There exists a cut $\prs{S^*,\overline{S^*}}$ 
such that $U\subset S^*$ and $U'\subset \overline{S^*}$
and has size at most 
\[
    \abs{E\prs{S^*,\overline{S^*}}}\leq \frac{m}{\gamma_{u,u'}(U,U')}
\]
where $\gamma_{u,u'}(U,U')==\frac{1}{3}\Reff(u,u')-\gamma_{eff}(U)
-\gamma_{eff}(U')$ and assume it to be strictly positive.
\end{lemma}

In our settings (and notation) 
we denote $\gamma_p(U)=\max_{x,y\in U}d_p(x,y)$.
Now,
we can use the same technique  from the proof of Lemma \ref{lemma: small cut from Madry} (with
minor changes)
in order to prove the following extension of it.
\begin{lemma}
Let $U,U'\subset V$ be disjoint sets in a graph $G$ having at most $m$
edges, let $p\in[1,\infty)$, let $u\in U$ and $u'\in U'$.
There exists a cut $\prs{S^*,\overline{S^*}}$ 
such that $U\subset S^*$ and $U'\subset \overline{S^*}$
and has size at most 
\[
    \abs{E\prs{S^*,\overline{S^*}}}\leq \frac{m^{1/p}}{\gamma_{u,u'}(U,U')}
\]
where $\gamma_{u,u'}(U,U')=d_p(u,u')-\gamma_{p}(U)
-\gamma_{p}(U')$ and assume it to be strictly positive.
\end{lemma}
\begin{proof}
Consider the graph $G'$ where we contracted the set of vertices of $U$
into a single vertex $u'$, as well as contracted $W$ into a single
vertex $w'$, and suppose that we removed self loops but kept parallel edges.
Suppose that the minimum $u'-w'$-cut in $G'$ is of size $k$.
Thus, there exists $k$ edge-disjoint paths in $G'$
that connect between $u'$ and $w'$.
This paths correspond to edge disjoint paths in the original graph $G$,
denote them by $\pi_1,\dots,\pi_k$, where each path $\pi_i$ begins in a vertex
$u_i\in U$ and ends in a vertex $w_i\in W$, and let $d_i$ be the length
of the $i$-th path.
We will now show that $d_p(u,w)\leq \gamma_p(U)+\gamma_p(W)+\frac{m^{1/p}}{k}$,
which will finish the proof.

For every $i$, denote  $f^*_{i,u}=\arg\min\curprs{\norm{W^{-1}f}_p
\,|\,f\in \R^m\text{ ships 1 unit of flow from }u\text{ to }u_i}$
and similarly
$f^*_{i,w}=\arg\min\curprs{\norm{W^{-1}f}_p
\,|\,f\in \R^m\text{ ships 1 unit of flow from }w_i\text{ to }w}$.
In other words, we chose $f_{i,u}^*$
such that $d_p\prs{u,u_i}=\norm{W^{-1}{f_{i,u}^*}}_p$,
and similarly for $f_{i,w}^*$ we have $d_p\prs{w_i,w}=\norm{W^{-1}{f_{i,w}^*}}_p$.
In addition, for every $i$, let $f_{\pi_i}=\Char_{\curprs{e\in\pi_i}}$
be a flow that ships 1 unit of flow from $u_i$ to $w_i$ along the path
$\pi_i$.
Finally, let $\widetilde{f}=\frac{1}{k}\sum_{i=1}^k\prs{f^*_{i,u}
+ f_{\pi_i} +f^*_{i,w} }$.
Note that $\widetilde{f}$ is a flow that ships 1 unit of flow from $u$
to $w$.
Thus we clearly have
\begin{equation}
    \begin{split}
        d_p(u,w)& \leq \norm{W^{-1}{\widetilde{f}}}_p\\
        & = \norm{\frac{1}{k}\sum_{i=1}^k\prs{W^{-1}{f^*_{i,u}}
            + W^{-1}{f_{\pi_i}} +W^{-1}{f^*_{i,w} }}}_p\\
        & \leq \frac{1}{k}\sum_{i=1}^k\norm{W^{-1}{f^*_{i,u}}}_p
        +\frac{1}{k}\norm{\sum_{i=1}^kW^{-1}{f^*_{\pi_i}}}_p
        +\frac{1}{k}\sum_{i=1}^k\norm{W^{-1}{f^*_{i,w}}}_p\\
        & \leq \frac{1}{k}\sum_{i=1}^k\gamma_p(U)
        +\frac{1}{k}\cdot m^{1/p}
        +\frac{1}{k}\sum_{i=1}^k\gamma_p(W)\\
        & =\gamma_p(U)+\gamma_p(W)+\frac{m^{1/p}}{k}
    \end{split}
\end{equation}
where we used the triangle inequality in the second transition.
Thus we conclude that
\begin{align*}
     d_p(u,w)-\prs{\gamma_p(U)+\gamma_p(W)}&\leq \frac{m^{1/p}}{k}\\
    \Rightarrow k&\leq \frac{m^{1/p}}{d_p(u,w)-\prs{\gamma_p(U)+\gamma_p(W)}}\\
\end{align*}
as claimed.


\end{proof}

\begin{claim}
Let $G=(V,E)$ be a graph with $m=|E|$ edges,
let $u,v\in V$ be some vertices,
and let $p\in[1,\infty)$.
Let 
$S^*\in \argmin{}\curprs{\abs{E\prs{S,\overline{S}}}
\,:\,S\subset V,v\in S,u\notin S}$.
Then
\[
    \Bar{d}_p^q(u,v)\leq 
    \abs{E\prs{S^*,\overline{S^*}}}\leq \frac{m^{1/p}}{d_p(v,u)}
\]
where $q$ is the H\"older conjugate of $p$.
\end{claim}
The proof is very similar to the above, for the RHS consider the 
(normalized) maxflow between $u$ and $v$.
For the LHS consider the indicator on the set $S^*$ as the potential.

We remark that this inequality is tight,
for example consider a graph with 2 vertices and $m$ parallel edges
of unit weight.
\end{comment}



